Generic Primitive Detection in Point Clouds Using Novel Minimal Quadric Fits

We present a novel and effective method for detecting 3D primitives in cluttered, unorganized point clouds, without axillary segmentation or type specification. We consider the quadric surfaces for encapsulating the basic building blocks of our environments - planes, spheres, ellipsoids, cones or cylinders, in a unified fashion. Moreover, quadrics allow us to model higher degree of freedom shapes, such as hyperboloids or paraboloids that could be used in non-rigid settings. We begin by contributing two novel quadric fits targeting 3D point sets that are endowed with tangent space information. Based upon the idea of aligning the quadric gradients with the surface normals, our first formulation is exact and requires as low as four oriented points. The second fit approximates the first, and reduces the computational effort. We theoretically analyze these fits with rigor, and give algebraic and geometric arguments. Next, by re-parameterizing the solution, we devise a new local Hough voting scheme on the null-space coefficients that is combined with RANSAC, reducing the complexity from $O(N^4)$ to $O(N^3)$ (three points). To the best of our knowledge, this is the first method capable of performing a generic cross-type multi-object primitive detection in difficult scenes without segmentation. Our extensive qualitative and quantitative results show that our method is efficient and flexible, as well as being accurate.

==> quadricbg12.tex <==
\section{Preliminaries}
\label{sec:description}
%\todo{Schematic overview of pipeline - I actually didn't want to put a pipeline image to this paper, for the first time :D But we can discuss.}
% \paragraph{Quadrics} % not needed as the section's name is "Quadrics"
%\begin{definition}
A quadric in 3D Euclidean space is a hypersurface defined by the zero set of a polynomial of degree two:
\begin{align}
\label{eq:quadric}
f (x,y,z)
&= Ax^2+ By^2 + Cz^2 + 2Dxy + 2Exz \\
& + 2Fyz + 2Gx + 2Hy + 2Iz + J = 0. \nonumber
\end{align}
%\end{definition}
%Equation (\ref{eq:quadric}) can be written in the vector form as the parameter-variable dot product $\vec{v}^T\vec{q} = 0$, with:
or similarly in the vector notation $\vec{v}^T\vec{q} = 0$ with:
\begin{align}
&\vec{q} = \begin{bmatrix}
           A & B & C & D & E & F & G & H & I & J
         \end{bmatrix}^T \\
&\vec{v} = \begin{bmatrix}
			x^2 & y^2 & z^2 & 2xy & 2xz & 2yz & 2x & 2y & 2z & 1
         \end{bmatrix}^T \nonumber
\end{align}
Using homogeneous coordinates, quadrics can be analyzed uniformly.
The point $\vec{x} = (x,y,z) \in \mathbb{R}^3$ lies on the quadric, if the projective algebraic equation over $\mathbb{RP}^3$ with $d_q(\vec{x}) := [\vec{x}^T  1]\vec{Q} [\vec{x}^T 1]^T$ holds true, where the matrix $\vec{Q} \in \mathbb{R}^{4 \times 4}$ is defined by re-arranging the coefficients:
\begin{equation}
\vec{Q} =
\SmallMatrix{
A & D & E & G\\
D & B & F & H\\
E & F & C & I\\
G & H & I & J
}
,\quad
\nabla \vec{Q} =  2
\SmallMatrix{
A & D & E & G \\
D & B & F & H \\
E & F & C & I
}.
\end{equation}
$d_q(\vec{x})$ can be viewed as an algebraic distance function. Similar to the quadric equation, the gradient at a given point can be written as $\nabla\vec{Q}(\vec{x}) := \nabla\vec{Q} [\vec{x}^T 1]^T$.
Quadrics are general implicit surfaces capable of representing cylinders, ellipsoids, cones, planes, hyperboloids, paraboloids and potentially the shapes interpolating any two of those.
All together there are 17 sub-types~\cite{Weisstein2017}.
Once $\vec{Q}$ is given, this type can be determined from an eigenvalue analysis of $\vec{Q}$ and its subspaces.
Note that quadrics have constant second order derivatives and are practically smooth.

A quadric whose matrix is of rank 2 consists of all points on a pair of planes.
It can be written as follows:
\[
\vec{Q} = \mathbf{\Pi}_1 \mathbf{\Pi}_2^T + \mathbf{\Pi}_2 \mathbf{\Pi}_1^T
\]
where $\Pi_1$ and $\Pi_2$ are the homogeneous 4-vectors representing the two planes. A quadric whose matrix is of rank 1 consists of a single plane.
It can be written as
\[
\vec{Q} = \mathbf{\Pi} \; \mathbf{\Pi}^T \enspace .
\]
\noindent The polar plane $\mathbf{\Pi}$ of a point $\vec{P}$ relative to a quadric $\vec{Q}$, is:
\[
\mathbf{\Pi} = \vec{Q} \vec{P} \enspace .
\]
Reciprocally, $\vec{P}$ is called the pole of plane $\vec{\Pi}$.
Note that if $\vec{Q} \vec{P} = \vec{0}$, then the polar plane does not exist for $\vec{P}$;
also note that for a point that lies on the quadric, the polar plane is the tangent plane in that point.

Some types of quadrics (ellipsoids, hyperboloids) are called central quadrics; they possess
a finite center point $\vec{c}$ that is the pole of the plane at infinity: $
\vec{Q} \vec{c} \sim \begin{bmatrix} 0 & 0 & 0 & 1 \end{bmatrix}^T$.
\]

\subsection{Dual Space}
Quadric dual space is formed by the Legendre transformation, mapping points to tangent planes as covectors. Every dual point represents a plane in the primal. Many operations such as fitting can be performed in either of the spaces~\cite{Cross1998}; or in the primal space using constraints of the dual. The latter forms a mixed primal-dual approach. Note that, knowing a point lies on the surface gives 1 constraint, and if, in addition, one knows the tangent plane at that point, then one gets 2 more constraints. This view will help to reduce the minimal point necessity, which Tab. \ref{tab:dualspace} summarizes for different mixes of primal and  dual spaces.

% Fitting a quadric can be performed in the primal space by using only 3D points, in the dual space using tangents or in a space composed of the blend of the two. This is obtained when the tangent plane is not independent, but rather anchored at a given point. We summarize the required minimal cases for the recovery of quadric in Table \ref{tab:dualspace}.

%\begin{table}[t!]
%  \centering
%  \caption{Minimal cases of quadric fitting. (PD: Primal/Dual)}
%    \begin{tabular}{lcccccc}
%          & Pri. & PD1 & PD2 & PD3 & PD4 & Dual \\
%    \toprule
%    {\# Points}  & 9 & 7 & 5 & 4 & 3 &1 \\
%    {\# Tangents}  & 0 & 1 & 2 &  & \\
%     \toprule
%    \end{tabular}%
%  \label{tab:dualspace}%
%\end{table}%


% \paragraph{Gradient of a Quadric}

%\begin{equation}
%\nabla \vec{Q} =  
%\begin{bmatrix}
%2A & D & E & G \\
%D & 2B & F & H \\
%E & F & 2C & I
%\end{bmatrix}
%\end{equation}


%\paragraph{Fitting of Quadric Surfaces}
%Fitting a quadric surface might seem trivial by using a least squares approach minimizing the squared distance function :
%\begin{equation}
%S=\sum\limits_{i=1}^N d_q(\vec{x}_i)^2
%\end{equation}
%To constrain the scale factor, Bronstein  proposed to use $\mathbf{\vec{a}^T\vec{a}=1}$. 

%\section{Distance between Quadrics}
%It is possible to define a correlation based distance term solely between the quadric coefficients:
%\begin{equation}
%\Gamma (Q_1, Q_2) = 1 - \abs*{ \frac{\sum\limits_{i=1}^{10} Q_{1,i}Q_{2,i}}{\sqrt{\sum\limits_{i=1}^{10} Q_{1,i}^2 Q_{2,i}^2}} }
%\end{equation}
%Indeed quadric blending techniques rely on the fact that two quadrics can be linearly interpolated to create and intermediary shape:
%\begin{equation}
%Q_{blend} = \lambda Q_1 + (1-\lambda)Q_2
%\end{equation}
%However, the probability distribution of quadric coefficients are highly non-linear. Therefore, similar quadrics give might rise to large distances, while distant quadrics can result in small $\Gamma (Q_1, Q_2)$ values. Therefore it is not appropriate to use such a straightforward measure.

